AutoChip: Automating HDL Generation Using LLM Feedback

Traditionally, designs are written in Verilog hardware description language (HDL) and debugged by hardware engineers. While this approach is effective, it is time-consuming and error-prone for complex designs. Large language models (LLMs) are promising in automating HDL code generation. LLMs are trained on massive datasets of text and code, and they can learn to generate code that compiles and is functionally accurate. We aim to evaluate the ability of LLMs to generate functionally correct HDL models. We build AutoChip by combining the interactive capabilities of LLMs and the output from Verilog simulations to generate Verilog modules. We start with a design prompt for a module and the context from compilation errors and debugging messages, which highlight differences between the expected and actual outputs. This ensures that accurate Verilog code can be generated without human intervention. We evaluate AutoChip using problem sets from HDLBits. We conduct a comprehensive analysis of the AutoChip using several LLMs and problem categories. The results show that incorporating context from compiler tools, such as Icarus Verilog, improves the effectiveness, yielding 24.20% more accurate Verilog. We release our evaluation scripts and datasets as open-source contributions at the following link https://github.com/shailja-thakur/AutoChip.

==> section/Approach.tex <==
\section{Proposed Method}

==> section/Evaluation.tex <==
\section{Evaluation}

% \begin{table*}
% \footnotesize

% \centering 
% \caption{Problems for evaluation}
% \begin{tabularx}{\textwidth}
% {|m{0.1\textwidth}|m{0.1\textwidth}|m{0.04\textwidth}|X|}
% \hline
% Difficulty & Category & Count & Problem Description \\ \hline
% % Getting Started & Getting Started & 2 & Getting Started, Output Zero \\ \hline
% \multirow{5}{*}{Verilog} & Basics & 8 & Simple/Four wires, Inverter, AND, NOR, XNOR, Declare wires, 7458 chip \\ \cline{2-4}
%  & Vectors & 9 & Vectors, Vectors (  detail), Vector part select, Bitwise operators, Four-input gates, Vector concatenate, Vector reversal 1, Replicate, More replication \\ \cline{2-4}
%  & Module Hierarchy & 9 & Modules, Connect ports by position, Connect ports by name, Three modules, Modules and vectors, Adder 1, Adder 2, Carry-select, Adder-subtractor \\ \cline{2-4}
%  & Procedures & 8 & Always blocks (combinational), Always blocks (clocked), If statement, If statement latches, Case statement, Priority encoder, Priority encoder with casez, Avoiding latches \\ \cline{2-4}
%  & More Features & 7 & Conditional ternary, Reduction operators, Reduction: Wider gates, Combinational for-loop: Vector reversal 2, Combination for-loop: 255-bit count, Generate for-loop: 100-bit adder 2, Generate for-loop: 100-digit BCD adder \\ \hline
% \multirow{4}{*}{Circuits} & Basic & 17 & Wire, GND, NOR, Another, Two gates, More gates, 7420 chip, Truth tables, Two-bit equality, Simple circuits A, B, Combine circuits A, B, Ring or vibrate?, Thermostat, 3-bit count, Gates and vectors, longer vectors \\ \cline{2-4}
% (Combination) & Multiplexers & 5 & 2-to-1 mux, 2-to-1 bus mux, 9-to-1 mux, 256-to-1 mux, 256-to-1 4-bit mux\\ \cline{2-4}
%  & Arithmetic Circuits & 7 & Half adder, Full adder, 3-bit adder, Signed addition overflow, 100-bit binary adder, 4-digit BCD adder \\ \cline{2-4}
%  & K-Map to Circuit & 8 & 3/4-variable, Minimum SOP and POS, K-map, K-map  with a mux \\ \hline
% \multirow{8}{*}{Circuits } & Latches and Flip-Flops & 18 & DFFs, DFF (reset), DFF (reset value), DFF (asynchronous), DFF (byte enable), D Latch, DFF,  DFF+gate, Mux and DFF, DFFs and gates, Circuit from truth table, Detect edge/both edges, Edge capture register, Dual-edge triggered FF \\ \cline{2-4}
% & Counters & 8 & Four-bit binary counter, Decade counter, Decade counter again, Slow decade counter, Counter 1-12, Counter 1000, 4-digit decimal counter, 12-hour clock \\ \cline{2-4}
%  (Sequential)  & Shift Registers & 9 & 4-bit shift register, Left/right rotator, Left/right arithmetic shift by 1 or 8, 5-bit LFSR, 3-bit LFSR, 32-bit LFSR, Shift register, Shift register, 3-input LUT \\ \cline{2-4}
%  & Cellular Automata & 3 & Rule 90, Rule 110, Conways Game of Life 16x16 \\ \cline{2-4}
%  & FSM & 33 & FSM 1 (asynchronous), FSM 1 (synchronous), FSM 2 (asynchronous), FSM 2 (synchronous), Simple state transitions 3, Simple one-hot state transition 3, FSM 3 (asynchronous), FSM 3 (synchronous), Moore FSM, Lemmings 1, Lemmings 2, Lemmings 3, Lemmings 4, One-hot FSM, PS/2 packet parser, PS/2 packet parser and datapath, Serial receiver, Serial receiver and datapath, Serial receiver with parity check, Sequence recognition, Q8: Design Mealy FSM, Q5a: Serial twos complementer (Moore FSM), Q5b: Serial twos complementer (Mealy FSM), Q2a, Q2b, Q3a, Q3b: FSM, Q3c: FSM logic, Q6b: FSM next-state logic, Q6c: FSM one-hot next-state logic, Q6: FSM, Q2a: FSM, Q2b: One-hot FSM equations  \\  \cline{2-4} 
%  & Larger Circuits & 7 & Counter with period 1000, 4-bit shift register and down counter, FSM: Sequence 1101 recognizer, FSM: Enable shift register, FSM: Complete FSM, Complete timer, FSM: One-hot logic equations \\ \hline
% Verify Bugs & Read Simulations \& Find bugs & 5 & Mux2, NAND, Mux4, Add/subtract, Case statement \\ \hline
% \end{tabularx}
% \label{tbl:problems-set-2}
% \end{table*}

















==> section/preamble/preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

\lstset{ 
%   escapeinside={(*@}{@*)},
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\scriptsize,        % the size of the fonts that are used for the code
  %breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
%   captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  %columns=fullflexible,
  keywordstyle=\color{blue},       % keyword style
  language=Verilog,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%   showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
%   tabsize=2,	                   % sets default tabsize to 2 spaces
%   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
%   %framesep=0pt,framerule=0pt,
%   %aboveskip=0pt,belowskip=0pt
    rulecolor=\color{black}
}



